Achieving Proportionality up to the Maximin Item with Indivisible Goods

We study the problem of fairly allocating indivisible goods and focus on the classic fairness notion of proportionality. The indivisibility of the goods is long known to pose highly non-trivial obstacles to achieving fairness, and a very vibrant line of research has aimed to circumvent them using appropriate notions of approximate fairness. Recent work has established that even approximate versions of proportionality (PROPx) may be impossible to achieve even for small instances, while the best known achievable approximations (PROP1) are much weaker. We introduce the notion of proportionality up to the maximin item (PROPm) and show how to reach an allocation satisfying this notion for any instance involving up to five agents with additive valuations. PROPm provides a well-motivated middle-ground between PROP1 and PROPx, while also capturing some elements of the well-studied maximin share (MMS) benchmark: another relaxation of proportionality that has attracted a lot of attention.

==> AverageEFx.tex <==
In addition to $\propXt$ we can consider a stronger notion of fairness called Average EFx or $\aEFx$. $\aEFx$ is a relation of EFx that requires every agent not envy every other agent on average after removing their least valuable item from their bundle. Formally we define an agent $i$ as being satisfied by $\aEFx$ is $\val{i}{i}>\frac{1}{n-1}\sum_{j\in N, j\neq i}(\val{i}{j}-d_{i}(X_j))$ where $d_i(X_j)$ is the value of $i$'s least valuable item in $j$'s bundle. Note $\propXt$ is strictly weaker than this where instead of subtracting $d_{i}(X_j)$ for each agent $j\neq i$ instead we subtract $\max_{j\neq i} d_i(X_j)$ for each agent $j\neq i$.

We seek to prove that an allocation where every agent is satisfied by $\aEFx$ always exists for additive valuations. In order to prove this, we defined a modified valuation function for each agent where $\adjVal{i}=\val{i}{i}+\frac{(n-1)}{n}d_{i}(X)$. If we normalize the agents' values for the entire set of items to 1, then if $\adjVal{i} \ge 1/n$, agent $i$ satisfied by $\aEFx$. 

\begin{lemma}
If $\adjVal{i} \ge 1/n$, agent $i$ satisfied by $\aEFx$.
\end{lemma}

We then consider all of the allocations in a leximin ordering where an allocation A is leximin dominated by allocation B if the agent with the lowest adjusted value in B is greater than the agent with the lowest adjusted value in A. Hence if we show that the agent with the lowest adjusted value in the leximin dominating allocation always has value greater than or equal to $1/n$ then an $\aEFx$ allocation is guaranteed to exist, but if the value is less than $1/n$ then that proves an $\aEFx$ allocation does not exist for that case. This would be a very result as that would imply no EFx allocation exists for that case since $\aEFx$ is strictly weaker than EFx. 

==> extraWork.tex <==

\section{Existence of PROPx}

We start with some simple properties of $\propXt$ comparing it to other versions of fairness. 

\begin{lemma}
If an allocation $X$ satisfies EFx then $X$ is $\propXt$.  
\end{lemma}

\begin{proof}
If an allocation $X$ satisfies EFx then $\val{i}{i} >\val{i}{j}-\minIn{i}{j} \ \forall j\in N$. Thus $\val{i}{i}>\frac{1}{n-1}\sum_{j\in N, j\neq i}(\val{i}{j}-\minIn{i}{j})> \frac{1}{n-1}\sum_{j\in N, j\neq i}(\val{i}{j}-d_{i}(X))$
\end{proof}

\begin{corollary}\label{noEFx=Propx}
If an agent $i$ does not EFx envy any other agents then $i$ is $\propXt$. 
\end{corollary}

\begin{lemma}\label{adjVal1}
If for an allocation $X$, $\adjVal{i}\geq 1$ then $i$ is $\propXt$ in $X$. 
\end{lemma}

\begin{proof}
$i$ is satisfied by $\propXt$ if
\begin{equation}\label{propXCondition}
\val{i}{i} > \frac{1}{n-1}\sum_{j\in N}\val{i}{j}-d_{i}(X)
\end{equation} We have 
\begin{align*}
\adjVal{i}=\val{i}{i}+\frac{n-1}{n}d_{i}(X) \geq 1 \Rightarrow \val{i}{i} > 1 - 
\frac{n-1}{n}d_{i}(X)
\end{align*}
Hence we get 
\begin{align*}
\sum_{j\in N, j\neq i}\val{i}{j} < n - 1 +\frac{n-1}{n}d_{i}(X) \Rightarrow \frac{1}{n-1}\sum_{j\in N, j\neq i}\val{i}{j} - d_{i}(X) < 1 + \frac{1-n}{n}d_{i}(X)
\end{align*}
 Thus we get $\val{i}{i} \ge 1 \ge \frac{1}{n-1}\sum_{j\in N, j\neq i}\val{i}{j} - d_{i}(X)$ and are done. 
\end{proof} 

\begin{corollary}\label{val1}
If for an allocation $X$, $\val{i}{i}>1-\frac{n-1}{n}m_{i}(M\setminus X_{i})$ then $i$ is $\propXt$ in $X$. 
\end{corollary}

One tool we use extensively is the leximin ordering over all the allocations as defined previously. Here we list some basic observations on it. 

\subsection{The Leximin Ordering}

\begin{theorem}
The leximin ordering defined according to $R\preceq S$ if $min_{i\in N}\tilde{v}_{i}(R)\le \tilde{v}_{i}(S)$ creates a total ordering over all possible allocations. 
\end{theorem}

\begin{proof}
To prove our ordering is a total ordering we must prove that for allocations $Q,R,S \subset 3^M$,
\begin{enumerate}
	\item $Q \prec Q$ is false 
	\item If $Q\preceq R$ and $R\preceq S$ then $Q\preceq S$. 
\end{enumerate}

(1): Start by ordering the adjusted values of all the agents according to their allocation in $Q$. Making 2 copies of this list shows that there are no differences between the agents' adjusted values so $Q=Q$ and $Q \prec Q$ is false. 

(2): If $Q\preceq R$ then $min_{i\in N}\tilde{v}_{i}(Q)\le min_{i\in N}\tilde{v}_{i}(R)$ for some $i$. If $R\preceq S$ then $min_{j\in N}\tilde{v}_{j}(R)\le min_{j\in N}\tilde{v}_{j}(S)$ for some $j$. If $i=j$ we are done as that means $Q$ and $S$ have the same adjusted values for all agents before $i$ and then $\tilde{v_{i}}(Q_{i})\le \tilde{v_{i}}(S_{i})$ making $Q\preceq S$. If $j\neq i$ then $R$ and $S$ must have had the same adjusted values for agents upto $j$. Thus $\tilde{v_{i}}(S_{i})=\tilde{v_{i}}(R_{i})\ge \tilde{v_{i}}(Q_{i})$ implying that $Q\preceq S$.
\end{proof}

\begin{corollary}
Since there are a finite amount of allocations, there exists a maximum allocation in the leximin ordering. 
\end{corollary}

\begin{lemma}\label{EFxCycleTrade}
If $X$ is the maximum allocation in the leximin ordering, then no cycles exist in $X$'s EFx envy graph.
\end{lemma}

\begin{proof}
Assume a cycle does exist in the EFx envy graph. We now show agents can trade bundles across the cycle for a leximin improvement. Call the allocation after swapping across the cycle $X^{\prime}$ Start by considering the agents outside of the cycle. They do not care who owns which bundle as long as the contents of the bundles stay the same. Thus their adjusted value remains constant throughout the swap. Now consider the agents inside the swap. WLOG consider agent $i$ who EFx envies $j$ giving away $X_{i}$ to recieve $X_{j}$ in the cycle swap. We look to show that
\begin{equation}\label{leximinImprovement}
\val{i}{j}+\frac{n-1}{n}d_{i}(X^{\prime})>\val{i}{i}+\frac{n-1}{n}d_{i}(X)
\end{equation}
 
There are 2 cases depending on whether $i$ is pointing towards $j$ in the $\propXt$ graph of $X.\newline$ 

Case 1: $d_{i}(X)$ is not defined by $X_{j}$

In this case $d_{i}(X)=d_{i}(X^{\prime})$. Thus all we need to show is that $\val{i}{j}>\val{i}{i}$. This is clear from the fact that $i$ EFx envied $j$. Thus $i$ sees a leximin improvement from the swap.$\newline$ 

Case 2: $d_{i}(X)$ is defined by $X_{j}$ 

In this case $d_{i}(X^{\prime})$ could equal 0, so we need to show that $\val{i}{j}>\val{i}{i}+\frac{n-1}{n}d_{i}(X)$. Since $i$ EFx envies $j$, we know that $\val{i}{j}-\minIn{i}{j}>\val{i}{i}$. Furthermore, since $d_{i}(X)$ is defined by $X_{j}$, $\minIn{i}{j}=d_{i}(X)$, so the previous inequality becomes $\val{i}{j}>\val{i}{i}+d_{i}(X)>\val{i}{i}+\frac{n-1}{n}d_{i}(X).\newline$

Since we arbitrarily chose $i$, every agent that is part of the swap saw a leximin improvement from swapping across the cycle. This contradicts the initial assumption that $X$ was already the maximum allocation in the leximin ordering, thus there must not be any cycles in the EFx envy graph.  
\end{proof}

Note that trading across cycles in the EF graph does not necessarily create a leximin improvement. This is because the values for $d_{i}(X)$ might be hurt more than an agent gains. 

From here, we move onto sufficient conditions for a $\propXt$ allocation to exist. 

\subsection{Sufficient Conditions}

\begin{theorem}\label{lessThan1}
If there exists an agent $i$ and a good $g$ such that $v_{i}(g)\ge 1$, then a $\propXt$ allocation exists. 
\end{theorem}

\begin{proof}
Assume otherwise. Then give the agent $i$ for which $v_{i}(g) \geq 1$ g. Now run the 2-Agent EFx algorithm on the other 2 agents over the remaining item. The agent who recieves the 1 item is satisfied by $\propXt$ since their adjusted value is above 1. Then the other 2 agents are satisfied since they don't EFx envy anyone. They don't EFx envy each other due to their bundles being allocated by the EFx algorithm, and they don't EFx envy the agent with 1 item since they remove that 1 item and see that agent as having 0 value. 
\end{proof}

We can extend this argument to larger bundles of goods as well. 

\begin{theorem}
If there exists a bundle $B$ such that $v_{i}(B) > 1 - \frac{2}{3}m_{i}(M\setminus B)$ and $v_{j}(B) - m_{j}(B)< \frac{v_j(M\setminus B)}{3} \ \forall j \neq i$ then a $\propXt$ solution exists.
\end{theorem}

\begin{proof}
Without loss of generality assume that agent $i$ is agent A, and we show that a $\propXt$ allocation exists using a constructive argument. We let $X_A=B$, i.e., we give agent 1 the bundle $B$, and we define $X_B$ and $X_C$ by computing an EFx allocation of the remaining items among agents B and C, i.e., an allocation such that $\val{B}{B}\geq \val{B}{C}-\minIn{B}{B}$ and $\val{C}{C}\geq \val{C}{B}-\minIn{C}{B}$. 

From Corollary ~\ref{val1}, we know that $A$ is satisfied by $\propXt$. 

In the rest of the proof, we show that the allocation described above also leads to a $\propXt$ allocation for agent B; symmetric arguments can be used to prove that the same is true for agent C as well. Formally, we prove the following inequality. 
\begin{equation}\label{ineq:PROPx}
v_B(X_B) \ge \frac{\val{B}{A}+\val{B}{C}-2d_{B}(X)}{2}  ~~\Longleftrightarrow~~ 2 v_B(X_B) \ge \val{B}{A}+\val{B}{C}-2d_{B}(X) .
\end{equation}

First, we use the fact, ${v}_B(B)-m_{B}(B)\le \frac{v_B(M\setminus B)}{3}$ and, 
thus, ${v}_B(X_A)-\minIn{B}{A}\le \frac{v_B(M\setminus X_A)}{3} = \frac{\val{B}{B}+\val{B}{C}}{3}$. 
Second, we use that $\val{B}{B}\geq \val{B}{C}-\minIn{B}{C}$, due to the fact that $X_B$ and $X_C$
were computed using an EFx algorithm, as discussed above.
These two facts, along with $d_{B}(X)=\max(\minIn{B}{A},\minIn{B}{C})$, reduce proving Inequality~\eqref{ineq:PROPx} to satisfying
\begin{equation}\label{ineq:PROPx2}
2 \val{B}{B} \ge \frac{\val{B}{B}+\val{B}{C}}{3}+\val{B}{B} ~~\Longleftrightarrow~~ \val{B}{B} \ge \frac{\val{B}{C}}{2}.
\end{equation}
Therefore, if $\val{B}{B} \ge \frac{\val{B}{C}}{2}$, then this allocation is PROPx. Also, note that
if $X_A$ contains less than two items, then $\val{B}{A}-\minIn{B}{A}=0$ and Inequality~\eqref{ineq:PROPx}
becomes $2 v_B(X_B) \ge v_B(X_C)-\minIn{B}{C}$, which is clearly satisfied since $v_B(X_B) \ge v_B(X_C)-\minIn{B}{C}$
by EFx between agents 2 and 3.

To conclude the proof, we focus on instances where $X_A$ contains at least two items and we show that 
Inequality~\eqref{ineq:PROPx2} is true for all such instances with valuations $v_{i}(g)< 1$. Which is the case or else we are done by Theorem ~\ref{lessThan1}.
In order to do so, we first observe that, since $X_A$ contains at least two items, 
$v_B(X_A)\leq 2v_B(X_A)-\minIn{B}{A}$, due to the fact that the least valuable item in $X_A$ from the
perspective of agent 2 cannot have more than half of the total value in $X_A$, i.e., $\minIn{B}{A}\leq v_B(X_A)/2$.
Combined with the fact that ${v}_B(X_A)-\minIn{B}{A}\le \frac{v_B(M\setminus X_A)}{3}$ (according to the theorem statement) and
the fact that $v_B(X_A)+v_B(X_B)+v_B(X_C)=3$, this implies that 
\begin{equation*}
v_B(X_B)+v_B(X_C) = 3-v_B(X_A) 
%\geq 3 -2({v}_B(X_A)-\minIn{B}{A}) 
\geq 3 - 2\frac{v_B(M\setminus X_A)}{3} 
= 3 - 2\frac{v_B(X_B)+v_B(X_C)}{3}
~~\Longrightarrow~~
v_B(X_B)+v_B(X_C) \geq \frac{9}{5}.
\end{equation*}

If Inequality~\eqref{ineq:PROPx2} is not satisfied, i.e., if $v_B(X_B) < \frac{v_B(X_C)}{2}$, then
the fact that $v_B(X_B)+v_B(X_C) \geq \frac{9}{5}$ implies that $v_B(X_C)>\frac{2}{3}\cdot \frac{9}{5}=\frac{6}{5}$.
Then $X_C$ must contain at least two items, otherwise its single item would have a value larger than 1.
Since $X_C$ contains at least two items, then $\minIn{B}{C}\leq v_B(X_C)/2$, i.e., the value of agent
2 for his least favorite item in $X_C$ can be no more than half of his value for all of $X_C$. This implies that
the adjusted value of agent 2 for $X_C$ is at least half of his actual value for it, i.e., $\val{B}{C}-\minIn{B}{C}\geq v_B(X_C)/2$. 
But, since $v_B(X_B)\geq {v}_B(X_C)-\minIn{B}{C}$, due to the EFx property between agents 2 and 3, these two inequalities
imply the desired $v_B(X_B) \ge \frac{v_B(X_C)}{2}$. 

\end{proof}

\begin{theorem}
If there exists a bundle $B$ such that $v_{i}(B) > 1 - \frac{2}{3}m_i(M\setminus B)$ , and  $v_{j}(B) < 1-\frac{p}{3} \ \forall j \neq i \in N$, where $v_{j}(g) < p \ \forall g \in M/B \ \forall j \neq i$ then a $\propXt$ solution exists.
\end{theorem}

\begin{proof}
Just as the previous theorem, we construct a $\propXt$ allocation.  WLOG assume the agent $i$ is $A$. Give $A$ $B$, and then run the 2-agent EFx algorithm to allocate the remaining items to $B$ and $C$. 

We know $A$ is satisfied by Lemma ~\ref{val1}.

It remains to show that $B$ and $C$ are satisfied by $\propXt$. We prove $B$ is satisfied, with the same argument following symmetrically for $C$. 

The theorem statement and our construction give us the following inequalities 
\begin{equation}\label{bundleThmEq1}
v_{B}(B)\le 1- \frac{p}{3}
\end{equation}
\begin{equation}\label{bundleThmEq2}
\val{B}{B}+\val{B}{C}=3-v_j(B)
\end{equation}
\begin{equation}\label{bundleThmEq3}
\val{B}{B}\ge \val{B}{C}-p
\end{equation}

We can then combine ~\eqref{bundleThmEq1} and ~\eqref{bundleThmEq2} to get 
\begin{equation}
\val{B}{B}+\val{B}{C}\ge 2 +\frac{p}{3} \Rightarrow 2\val{B}{B}\ge 2-\frac{2p}{3} \Rightarrow \val{B}{B}\ge 1-\frac{p}{3}
\end{equation}

Thus $\val{B}{B} \ge \val{B}{A}-\minIn{B}{A}$ and $\val{B}{C} \ge \val{B}{A}-\minIn{B}{C}$. So $B$ does not EFx envy anyone and is hence satisfied by $\propXt$. 

\end{proof}

\begin{corollary}
If there exists a bundle $B$ such that $v_{i}(B) > 1 - \frac{2}{3}m_i(M\setminus B)$ , and if $v_{j}(B)-m_{j}(B) < 1-\frac{p+\sigma}{3} \ \forall j \neq i \in N$, where $v_{j}(g) < p \ \forall g \in M/B \ \forall j \neq i$, and $v_{j}(g) \leq \sigma \ \forall g \in B \ \forall j \neq i$ then a $\propXt$ solution exists.
\end{corollary}

\begin{proof}
The proof follows exactly the same as the previous theorem, just adding in a $\sigma$ and subtracting $m_{j}(B)$ wherever applicable. 
\end{proof}



==> techniques.tex <==
To prove the existence of $\propXt$ we use a leximin ordering. Since there are a finite number of possible allocations, it is possible to define a total ordering on them according to maximizing the minimum adjusted $\propXt$ value over all the agents in a given allocation. We precisely define this ordering below. We show that if a given allocation does not satisfy $\propXt$  then there exists some swap towards a leximin improved allocation according to the ordering. Thus, the allocation at the top of the leximin ordering must be satisfied by $\propXt$. The exact nature of which swap is used towards a leximin improvement varies widely and is mostly done on the basis of casework. 
